Effect Heterogeneity with Earth Observation in Randomized Controlled Trials: Exploring the Role of Data, Model, and Evaluation Metric Choice

Many social and environmental phenomena are associated with macroscopic changes in the built environment, captured by satellite imagery on a global scale and with daily temporal resolution. While widely used for prediction, these images and especially image sequences remain underutilized for causal inference, especially in the context of randomized controlled trials (RCTs), where causal identification is established by design. In this paper, we develop and compare a set of general tools for analyzing Conditional Average Treatment Effects (CATEs) from temporal satellite data that can be applied to any RCT where geographical identifiers are available. Through a simulation study, we analyze different modeling strategies for estimating CATE in sequences of satellite images. We find that image sequence representation models with more parameters generally yield a greater ability to detect heterogeneity. To explore the role of model and data choice in practice, we apply the approaches to two influential RCTs -- Banerjee et al. (2015), a poverty study in Cusco, Peru, and Bolsen et al. (2014), a water conservation experiment in Georgia, USA. We benchmark our image sequence models against image-only, tabular-only, and combined image-tabular data sources, summarizing practical implications for investigators in a multivariate analysis. Land cover classifications over satellite images facilitate interpretation of what image features drive heterogeneity. We also show robustness to data and model choice of satellite-based generalization of the RCT results to larger geographical areas outside the original. Overall, this paper shows how satellite sequence data can be incorporated into the analysis of RCTs, and provides evidence about the implications of data, model, and evaluation metric choice for causal analysis.

==> CompMat_Georgia.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Mon, Jun 10, 2024 - 12:58:45
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Georgia analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $1.258$ & $1.301$ \\ 
EO+Tabular & $1.494$ & $2.341$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_Joint.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Jun 22, 2024 - 07:44:46
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Georgia, joint analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.038$ & $0.223$ \\ 
EO+Tabular & $0.061$ & $0.500$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_Joint_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{Joint ratio. Georgia, joint analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.126$ & $0.397$ \\ 
EO+Tabular & $0.221$ & $0.626$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_Joint_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with Joint weighting. Georgia, joint analysis. 
                                                               } 
  \label{tab:SumTab_GeorgiaJoint_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.835$ & $0.794$ \\ 
EO+Tabular & $0.708$ & $0.972$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_Joint_Joint.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:16:06
\begin{table}[!htbp] \centering 
  \caption{Joint ratio. Georgia, joint analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.177$ & $0.371$ \\ 
EO+Tabular & $0.188$ & $0.554$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_Joint_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{Joint ratio. Georgia, joint analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.173$ & $0.398$ \\ 
EO+Tabular & $0.198$ & $0.580$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_Joint_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with Joint weighting. Georgia, joint analysis. 
                                                               } 
  \label{tab:SumTab_GeorgiaJoint_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.695$ & $0.671$ \\ 
EO+Tabular & $0.585$ & $0.864$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_image.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Jun 22, 2024 - 07:44:46
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Georgia, image analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $$-$0.019$ & $0.417$ \\ 
EO+Tabular & $$-$0.111$ & $0.505$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_image_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{image ratio. Georgia, image analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $$-$0.117$ & $0.278$ \\ 
EO+Tabular & $0.060$ & $0.494$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_image_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with image weighting. Georgia, image analysis. 
                                                               } 
  \label{tab:SumTab_Georgiaimage_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.755$ & $0.637$ \\ 
EO+Tabular & $0.536$ & $0.793$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_image_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{image ratio. Georgia, image analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.026$ & $0.283$ \\ 
EO+Tabular & $$-$0.017$ & $0.578$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_image_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with image weighting. Georgia, image analysis. 
                                                               } 
  \label{tab:SumTab_Georgiaimage_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.580$ & $0.326$ \\ 
EO+Tabular & $0.354$ & $0.653$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_image_image.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:16:06
\begin{table}[!htbp] \centering 
  \caption{image ratio. Georgia, image analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $$-$0.057$ & $0.283$ \\ 
EO+Tabular & $$-$0.098$ & $0.382$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_video.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Jun 22, 2024 - 07:44:46
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Georgia, video analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $$-$0.131$ & $$-$0.052$ \\ 
EO+Tabular & $$-$0.012$ & $0.431$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_video_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{video ratio. Georgia, video analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.184$ & $0.352$ \\ 
EO+Tabular & $0.232$ & $0.637$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_video_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with video weighting. Georgia, video analysis. 
                                                               } 
  \label{tab:SumTab_Georgiavideo_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.849$ & $0.812$ \\ 
EO+Tabular & $0.769$ & $1.044$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_video_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{video ratio. Georgia, video analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.172$ & $0.337$ \\ 
EO+Tabular & $0.254$ & $0.465$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_video_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with video weighting. Georgia, video analysis. 
                                                               } 
  \label{tab:SumTab_Georgiavideo_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.722$ & $0.807$ \\ 
EO+Tabular & $0.684$ & $0.933$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Georgia_video_video.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:16:06
\begin{table}[!htbp] \centering 
  \caption{video ratio. Georgia, video analysis. 
                                                               } 
  \label{tab:SumTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.184$ & $0.352$ \\ 
EO+Tabular & $0.232$ & $0.637$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Mon, Jun 10, 2024 - 12:58:45
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Joint analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.433$ & $0.864$ \\ 
EO+Tabular & $0.737$ & $1.067$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_Joint.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Jun 22, 2024 - 07:44:46
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Joint, joint analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.056$ & $0.120$ \\ 
EO+Tabular & $0.046$ & $0.173$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_Joint_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{Joint ratio. Joint, joint analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.659$ & $0.723$ \\ 
EO+Tabular & $0.688$ & $0.823$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_Joint_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with Joint weighting. Joint, joint analysis. 
                                                               } 
  \label{tab:SumTab_JointJoint_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.917$ & $0.843$ \\ 
EO+Tabular & $0.863$ & $0.949$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_Joint_Joint.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:16:06
\begin{table}[!htbp] \centering 
  \caption{Joint ratio. Joint, joint analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.047$ & $0.223$ \\ 
EO+Tabular & $0.058$ & $0.279$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_Joint_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{Joint ratio. Joint, joint analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.551$ & $0.648$ \\ 
EO+Tabular & $0.546$ & $0.738$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_Joint_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with Joint weighting. Joint, joint analysis. 
                                                               } 
  \label{tab:SumTab_JointJoint_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.776$ & $0.663$ \\ 
EO+Tabular & $0.730$ & $0.780$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_image.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Jun 22, 2024 - 07:44:46
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Joint, image analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $$-$0.028$ & $0.283$ \\ 
EO+Tabular & $$-$0.096$ & $0.220$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_image_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{image ratio. Joint, image analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.589$ & $0.805$ \\ 
EO+Tabular & $0.657$ & $0.860$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_image_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with image weighting. Joint, image analysis. 
                                                               } 
  \label{tab:SumTab_Jointimage_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.927$ & $0.792$ \\ 
EO+Tabular & $0.833$ & $0.877$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_image_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{image ratio. Joint, image analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.481$ & $0.693$ \\ 
EO+Tabular & $0.432$ & $0.799$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_image_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with image weighting. Joint, image analysis. 
                                                               } 
  \label{tab:SumTab_Jointimage_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.740$ & $0.490$ \\ 
EO+Tabular & $0.642$ & $0.662$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_image_image.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:16:06
\begin{table}[!htbp] \centering 
  \caption{image ratio. Joint, image analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $$-$0.159$ & $0.191$ \\ 
EO+Tabular & $$-$0.161$ & $0.202$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_video.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Jun 22, 2024 - 07:44:46
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Joint, video analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.046$ & $$-$0.061$ \\ 
EO+Tabular & $0.081$ & $0.095$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_video_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{video ratio. Joint, video analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.788$ & $0.707$ \\ 
EO+Tabular & $0.791$ & $0.864$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_video_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with video weighting. Joint, video analysis. 
                                                               } 
  \label{tab:SumTab_Jointvideo_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $1.004$ & $0.940$ \\ 
EO+Tabular & $0.970$ & $1.084$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_video_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{video ratio. Joint, video analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.629$ & $0.631$ \\ 
EO+Tabular & $0.658$ & $0.726$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_video_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with video weighting. Joint, video analysis. 
                                                               } 
  \label{tab:SumTab_Jointvideo_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.848$ & $0.802$ \\ 
EO+Tabular & $0.834$ & $0.899$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Joint_video_video.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:16:06
\begin{table}[!htbp] \centering 
  \caption{video ratio. Joint, video analysis. 
                                                               } 
  \label{tab:SumTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.145$ & $0.223$ \\ 
EO+Tabular & $0.164$ & $0.325$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Mon, Jun 10, 2024 - 12:58:45
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Peru analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $$-$0.392$ & $0.428$ \\ 
EO+Tabular & $$-$0.021$ & $$-$0.207$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_Joint.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Jun 22, 2024 - 07:44:46
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Peru, joint analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.073$ & $0.016$ \\ 
EO+Tabular & $0.032$ & $$-$0.155$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_Joint_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{Joint ratio. Peru, joint analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $1.191$ & $1.048$ \\ 
EO+Tabular & $1.155$ & $1.020$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_Joint_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with Joint weighting. Peru, joint analysis. 
                                                               } 
  \label{tab:SumTab_PeruJoint_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.999$ & $0.892$ \\ 
EO+Tabular & $1.017$ & $0.926$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_Joint_Joint.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:16:06
\begin{table}[!htbp] \centering 
  \caption{Joint ratio. Peru, joint analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $$-$0.083$ & $0.075$ \\ 
EO+Tabular & $$-$0.073$ & $0.004$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_Joint_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{Joint ratio. Peru, joint analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.928$ & $0.898$ \\ 
EO+Tabular & $0.894$ & $0.896$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_Joint_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with Joint weighting. Peru, joint analysis. 
                                                               } 
  \label{tab:SumTab_PeruJoint_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.858$ & $0.655$ \\ 
EO+Tabular & $0.875$ & $0.696$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_image.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Jun 22, 2024 - 07:44:46
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Peru, image analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $$-$0.036$ & $0.148$ \\ 
EO+Tabular & $$-$0.081$ & $$-$0.064$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_image_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{image ratio. Peru, image analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $1.295$ & $1.332$ \\ 
EO+Tabular & $1.255$ & $1.227$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_image_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with image weighting. Peru, image analysis. 
                                                               } 
  \label{tab:SumTab_Peruimage_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $1.099$ & $0.946$ \\ 
EO+Tabular & $1.130$ & $0.961$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_image_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{image ratio. Peru, image analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.936$ & $1.103$ \\ 
EO+Tabular & $0.882$ & $1.020$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_image_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with image weighting. Peru, image analysis. 
                                                               } 
  \label{tab:SumTab_Peruimage_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.900$ & $0.654$ \\ 
EO+Tabular & $0.930$ & $0.671$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_image_image.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:16:06
\begin{table}[!htbp] \centering 
  \caption{image ratio. Peru, image analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $$-$0.261$ & $0.099$ \\ 
EO+Tabular & $$-$0.224$ & $0.021$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_video.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Jun 22, 2024 - 07:44:46
\begin{table}[!htbp] \centering 
  \caption{AUTOC ratio. Peru, video analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.222$ & $$-$0.070$ \\ 
EO+Tabular & $0.175$ & $$-$0.242$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_video_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{video ratio. Peru, video analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $1.393$ & $1.063$ \\ 
EO+Tabular & $1.350$ & $1.091$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_video_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with video weighting. Peru, video analysis. 
                                                               } 
  \label{tab:SumTab_Peruvideo_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $1.160$ & $1.068$ \\ 
EO+Tabular & $1.171$ & $1.124$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_video_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 22:03:48
\begin{table}[!htbp] \centering 
  \caption{video ratio. Peru, video analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $1.087$ & $0.924$ \\ 
EO+Tabular & $1.062$ & $0.987$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_video_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{RATE ratio with video weighting. Peru, video analysis. 
                                                               } 
  \label{tab:SumTab_Peruvideo_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw EO Space & EO PCs \\ 
\hline \\[-1.8ex] 
EO & $0.973$ & $0.797$ \\ 
EO+Tabular & $0.984$ & $0.866$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> CompMat_Peru_video_video.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:16:06
\begin{table}[!htbp] \centering 
  \caption{video ratio. Peru, video analysis. 
                                                               } 
  \label{tab:SumTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
EO & $0.106$ & $0.094$ \\ 
EO+Tabular & $0.096$ & $0.013$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> FULL_tabRATERatioRegs_SEanalytical.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Wed, Jul 24, 2024 - 09:12:42
\begin{footnotesize}
                                                            \begin{longtable}{lcc}  
  \caption{Outcome: RATE ratio. } 
  \label{tab:FULL_RegRATERatioRegs_SEanalytical} 
\footnotesize 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Model 1 & Model 2 \\ 
\hline \\[-1.8ex] 
\endfirsthead
\multicolumn{3}{c}
{\it (Continued from previous page)} \\
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Model 1 & Model 2 \\ 
\hline \\[-1.8ex] 
\endhead
 Video (Baseline:  Image) & 0.23 (NaN.00) & 0.09 (NaN.00) \\ 
 Transformer? (Baseline:  C N N) & 0.04 (NaN.00) &  \\ 
 Model,  Random proj (Baseline:  Clay) & -0.28 (NaN.00) &  \\ 
optimize Image Repvideomae-base & -0.48 (NaN.00) &  \\ 
optimize Image Repvit-base & -0.07 (NaN.00) &  \\ 
 With Tabular T R U E & -0.06 (NaN.00) & -0.06 (NaN.00) \\ 
 With Q T R U E & -0.18 (NaN.00) & -0.18 (NaN.00) \\ 
 With P C T R U E & -0.12 (NaN.00) & -0.12 (NaN.00) \\ 
application Peru & 0.32 (NaN.00) & 0.32 (NaN.00) \\ 
 I(log(1 + f2n(n Params Rep))) &  & 0.04 (NaN.00) \\ 
 Adjusted  R-squared & 0.31 & 0.23 \\ 
 Observations & 108 & 108 \\ 
 Countries & Error in eval(parse(text = evalTex\_nSuperunits))[row.names(my\_lm\$model),  : 
  Can't subset columns that don't exist.
[31m✖[39m Column `country` doesn't exist.
 & Error in eval(parse(text = evalTex\_nSuperunits))[row.names(my\_lm\$model),  : 
  Can't subset columns that don't exist.
[31m✖[39m Column `country` doesn't exist.
 \\ 
\hline \\[-1.8ex] 
 
\end{longtable}
                                                            \end{footnotesize} 


==> LandCors_Georgia_Joint.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:39:43
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, joint analysis. 
                                                               } 
  \label{tab:LandCorsTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.229$ & $0.203$ \\ 
R-squared & $$-$0.398$ & $$-$0.123$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_Joint_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, joint analysis. 
                                                               } 
  \label{tab:LandCorsTab_Georgia_Joint_} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.229$ & $0.203$ \\ 
R-squared & $$-$0.398$ & $$-$0.123$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_Joint_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, joint analysis. AUTOC weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Georgia_Joint_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.130$ & $0.089$ \\ 
RATE Ratio & $0.486$ & $0.043$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_Joint_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, joint analysis. 
                                                               } 
  \label{tab:LandCorsTab_Georgia_Joint_Q} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.229$ & $0.203$ \\ 
R-squared & $0.073$ & $0.105$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_Joint_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, joint analysis. QINI weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Georgia_Joint_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.130$ & $0.089$ \\ 
RATE Ratio & $0.095$ & $0.039$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_image.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:39:43
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, image analysis. 
                                                               } 
  \label{tab:LandCorsTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.289$ & $0.281$ \\ 
R-squared & $$-$0.978$ & $$-$0.732$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_image_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, image analysis. 
                                                               } 
  \label{tab:LandCorsTab_Georgia_image_} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.289$ & $0.281$ \\ 
R-squared & $$-$0.978$ & $$-$0.732$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_image_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, image analysis. AUTOC weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Georgia_image_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.130$ & $0.089$ \\ 
RATE Ratio & $0.486$ & $0.043$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_image_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, image analysis. 
                                                               } 
  \label{tab:LandCorsTab_Georgia_image_Q} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.289$ & $0.281$ \\ 
R-squared & $0.073$ & $0.105$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_image_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, image analysis. QINI weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Georgia_image_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.130$ & $0.089$ \\ 
RATE Ratio & $0.095$ & $0.039$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_video.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:39:43
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, video analysis. 
                                                               } 
  \label{tab:LandCorsTab_Georgia} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.193$ & $0.156$ \\ 
R-squared & $$-$0.050$ & $0.243$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_video_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, video analysis. 
                                                               } 
  \label{tab:LandCorsTab_Georgia_video_} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.193$ & $0.156$ \\ 
R-squared & $$-$0.050$ & $0.243$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Georgia_video_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Georgia, video analysis. 
                                                               } 
  \label{tab:LandCorsTab_Georgia_video_Q} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.193$ & $0.156$ \\ 
R-squared & $0.073$ & $0.105$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_Joint.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:39:43
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, joint analysis. 
                                                               } 
  \label{tab:LandCorsTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.229$ & $0.203$ \\ 
R-squared & $$-$0.398$ & $$-$0.123$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_Joint_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, joint analysis. 
                                                               } 
  \label{tab:LandCorsTab_Joint_Joint_} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.229$ & $0.203$ \\ 
R-squared & $$-$0.398$ & $$-$0.123$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_Joint_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, joint analysis. AUTOC weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Joint_Joint_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.175$ & $0.150$ \\ 
RATE Ratio & $0.465$ & $0.265$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_Joint_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, joint analysis. 
                                                               } 
  \label{tab:LandCorsTab_Joint_Joint_Q} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.229$ & $0.203$ \\ 
R-squared & $$-$0.117$ & $$-$0.037$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_Joint_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, joint analysis. QINI weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Joint_Joint_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.175$ & $0.150$ \\ 
RATE Ratio & $0.095$ & $0.038$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_image.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:39:43
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, image analysis. 
                                                               } 
  \label{tab:LandCorsTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.289$ & $0.281$ \\ 
R-squared & $$-$0.978$ & $$-$0.732$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_image_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, image analysis. 
                                                               } 
  \label{tab:LandCorsTab_Joint_image_} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.289$ & $0.281$ \\ 
R-squared & $$-$0.978$ & $$-$0.732$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_image_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, image analysis. AUTOC weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Joint_image_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.175$ & $0.150$ \\ 
RATE Ratio & $0.465$ & $0.265$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_image_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, image analysis. 
                                                               } 
  \label{tab:LandCorsTab_Joint_image_Q} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.289$ & $0.281$ \\ 
R-squared & $$-$0.117$ & $$-$0.037$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_image_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, image analysis. QINI weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Joint_image_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.175$ & $0.150$ \\ 
RATE Ratio & $0.095$ & $0.038$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_video.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:39:43
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, video analysis. 
                                                               } 
  \label{tab:LandCorsTab_Joint} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.193$ & $0.156$ \\ 
R-squared & $$-$0.050$ & $0.243$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_video_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, video analysis. 
                                                               } 
  \label{tab:LandCorsTab_Joint_video_} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.193$ & $0.156$ \\ 
R-squared & $$-$0.050$ & $0.243$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_video_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, video analysis. AUTOC weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Joint_video_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.175$ & $0.150$ \\ 
RATE Ratio & $0.465$ & $0.265$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_video_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, video analysis. 
                                                               } 
  \label{tab:LandCorsTab_Joint_video_Q} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.193$ & $0.156$ \\ 
R-squared & $$-$0.117$ & $$-$0.037$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Joint_video_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Joint, video analysis. QINI weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Joint_video_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.175$ & $0.150$ \\ 
RATE Ratio & $0.095$ & $0.038$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_Joint.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:39:43
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, joint analysis. 
                                                               } 
  \label{tab:LandCorsTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.229$ & $0.203$ \\ 
R-squared & $$-$0.398$ & $$-$0.123$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_Joint_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, joint analysis. 
                                                               } 
  \label{tab:LandCorsTab_Peru_Joint_} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.229$ & $0.203$ \\ 
R-squared & $$-$0.398$ & $$-$0.123$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_Joint_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, joint analysis. AUTOC weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Peru_Joint_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.219$ & $0.211$ \\ 
RATE Ratio & $0.443$ & $0.486$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_Joint_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, joint analysis. 
                                                               } 
  \label{tab:LandCorsTab_Peru_Joint_Q} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.229$ & $0.203$ \\ 
R-squared & $$-$0.308$ & $$-$0.179$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_Joint_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, joint analysis. QINI weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Peru_Joint_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.219$ & $0.211$ \\ 
RATE Ratio & $0.094$ & $0.038$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_image.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:39:43
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, image analysis. 
                                                               } 
  \label{tab:LandCorsTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.289$ & $0.281$ \\ 
R-squared & $$-$0.978$ & $$-$0.732$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_image_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, image analysis. 
                                                               } 
  \label{tab:LandCorsTab_Peru_image_} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.289$ & $0.281$ \\ 
R-squared & $$-$0.978$ & $$-$0.732$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_image_AUTOC.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, image analysis. AUTOC weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Peru_image_AUTOC} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.219$ & $0.211$ \\ 
RATE Ratio & $0.443$ & $0.486$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_image_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, image analysis. 
                                                               } 
  \label{tab:LandCorsTab_Peru_image_Q} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.289$ & $0.281$ \\ 
R-squared & $$-$0.308$ & $$-$0.179$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_image_QINI.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jul 23, 2024 - 17:59:47
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and RATE ratio (mean/std),  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, image analysis. QINI weighting method in RATE calculation.
                                                               } 
  \label{tab:LandCorsTab_Peru_image_QINI} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.219$ & $0.211$ \\ 
RATE Ratio & $0.094$ & $0.038$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_video.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:39:43
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, video analysis. 
                                                               } 
  \label{tab:LandCorsTab_Peru} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.193$ & $0.156$ \\ 
R-squared & $$-$0.050$ & $0.243$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_video_.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, video analysis. 
                                                               } 
  \label{tab:LandCorsTab_Peru_video_} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.193$ & $0.156$ \\ 
R-squared & $$-$0.050$ & $0.243$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> LandCors_Peru_video_Q.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Tue, Jun 25, 2024 - 08:53:28
\begin{table}[!htbp] \centering 
  \caption{Land cover comparisions, average correlation and AUTOC ratio,  
                                                                average taken across the set of image sequence modeling strategies. 
                                                                Peru, video analysis. 
                                                               } 
  \label{tab:LandCorsTab_Peru_video_Q} 
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Raw Space & PCs \\ 
\hline \\[-1.8ex] 
Correlation & $0.193$ & $0.156$ \\ 
R-squared & $$-$0.308$ & $$-$0.179$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 

